Network-Wide Task Offloading With LEO Satellites: A Computation and Transmission Fusion Approach

Computing tasks are ubiquitous in space missions. Conventionally, these tasks are offloaded to ground servers for computation, where the transmission of raw data on satellite-to-ground links severely constrains the performance. To overcome this limitation, recent works offload tasks to visible low-earth-orbit (LEO) satellites. However, this offloading scheme is difficult to achieve good performance in actual networks with uneven loads because visible satellites over hotspots tend to be overloaded. Therefore, it is urgent to extend the offloading targets to the entire network. To address the network-wide offloading problem, we propose a metagraph-based computation and transmission fusion offloading scheme for multi-tier networks. Specifically, virtual edges, between the original network and its duplicate, are generated to fuse computation and transmission in single-tier networks. Then, a metagraph is employed to integrate the fusion in multi-tier networks. After assigning appropriate edge weights to the metagraph, the network-wide offloading problem can be solved by searching the shortest path. In addition, we apply the proposed scheme to solve the spatial computation offloading problem in a real multi-tier network. The superiority of the proposed scheme over two benchmark schemes are proved theoretically and empirically. Simulation results show that the proposed scheme decreases the weighted average delay by up to 87.51% and 18.70% compared with the ground offloading scheme and the visible offloading scheme, respectively.

==> 1-Latex - arxiv/Sentence.tex <==
In addition to industry growing interest, academic
researchers have eagerly jumped into the development of small
satellites.

However, despite of great potential of FSO communication, its performance is limited by the adverse effects (viz., absorption, scattering, and turbulence) of the atmospheric channel. Out of these three effects, the atmospheric turbulence is a major challenge that may lead to serious degradation in the bit error rate performance of the system and make the communication link infeasible~\cite{7553489}. 

RS techniques have opened a door to helping people widen their ability to understand the earth [1], [2]. In fact, RS techniques are becoming more and more important in data-collection tasks. Information technology companies depend on RS to update their location-based services [3], [4]. Google Earth employs high-resolution (HR) RS images to provide vivid pictures of the earth s surface. Governments have also utilized RS for a variety of public services, from weather reporting to traffic monitoring [5] [7]. Nowadays, one cannot imagine a life without RS. Recent years have even witnessed a boom in RS satellites, providing for the first time an extremely large number of geographical images of nearly every corner of the earth s  surface [8]. Data warehouses of RS images are increasing daily, including images with different spectral and spatial resolutions [9], [10]. ~\cite{7486259}

==> 1-Latex - arxiv/table1.tex <==
%
\begin{tabular}{cccc} 
	%\toprule
	\rowcolor[rgb]{0.812,0.835,0.918} Product             & Processor                                                                                                                  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Computing\\Capability\end{tabular} & Reference                                     \\
	Xiphos
	
	Q7S                                           & Xilinx Zynq 7020                                                                                                           & 180                                                                                                & \cite{XiphosQ7S}                              \\
	\rowcolor[rgb]{0.914,0.922,0.961} Xiphos Q8S          & Xilinx Ultrascale+                                                                                                         & 1800                                                                                               & \cite{XiphosQ8S}                              \\
	BAE RAD5545                                           & RAD5545                                                                                                                    & 3.7                                                                                                & \cite{BAERAD5545}                             \\
	\rowcolor[rgb]{0.914,0.922,0.961} Innoflight CFC-500  & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.914,0.922,0.961}}c@{}}Xilinx Kintex Ultrascale+, \\NVIDIA TK1\end{tabular}       & 1290                                                                                               & \cite{CFC500}                                 \\
	MOOG G-Series Steppe Eagle                            & AMD G-Series compatible                                                                                                    & 75                                                                                                 & \cite{MOOG}                                   \\
	\rowcolor[rgb]{0.914,0.922,0.961} MOOG V-Series Ryzen & AMD V-Series compatible                                                                                                    & 1000                                                                                               & \cite{MOOG}                                   \\
	Unibap iX5-100                                        & \begin{tabular}[c]{@{}c@{}}Microchip SmartFusion2,\\AMD G-Series SOC\end{tabular}                                          & 127                                                                                                & \cite{iX5-100,bruhn2020enabling}              \\
	\rowcolor[rgb]{0.914,0.922,0.961} Unibap iX10-100     & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.914,0.922,0.961}}c@{}}Microchip PolarFire, \\AMD V1605b (Ryzen)\end{tabular}     & 3600                                                                                               & \cite{iX10-100,bruhn2020enabling}             \\
	SpaceCube v2.0                                        & Xilinx Virtex 5                                                                                                            & 200                                                                                                & \cite{SpaceCube2.0}                           \\
	\rowcolor[rgb]{0.914,0.922,0.961} SpaceCube v3.0      & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.914,0.922,0.961}}c@{}}Xilinx Kintex UltraScale,\\ Xilinx Zynq MPSoC\end{tabular} & 590                                                                                                & \cite{geist2019spacecube,SpaceCube3.0Patent}  \\
	%\bottomrule
\end{tabular}

==> 1-Latex - arxiv/table2-new.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
	\hline
	\rowcolor[rgb]{0.812,0.835,0.918} {\cellcolor[rgb]{0.812,0.835,0.918}}                            & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                       & {\cellcolor[rgb]{0.812,0.835,0.918}}                           & \multicolumn{3}{c|}{Offloading Target}                                                                                                                                                                                                                             & \multicolumn{3}{c|}{Optimization}                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ 
	\hhline{|>{\arrayrulecolor[rgb]{0.812,0.835,0.918}}--->{\arrayrulecolor{black}}------|}
	\rowcolor[rgb]{0.812,0.835,0.918} {\cellcolor[rgb]{0.812,0.835,0.918}}                            & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                       & {\cellcolor[rgb]{0.812,0.835,0.918}}                           & {\cellcolor[rgb]{0.812,0.835,0.918}}                         & \multicolumn{2}{c|}{Space}                                                                                                                                                                          & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                    & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                       & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                    \\ 
	\hhline{|>{\arrayrulecolor[rgb]{0.812,0.835,0.918}}---->{\arrayrulecolor{black}}-->{\arrayrulecolor[rgb]{0.812,0.835,0.918}}--->{\arrayrulecolor{black}}|}
	\rowcolor[rgb]{0.812,0.835,0.918} \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Reference} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Network\\~Architechture\end{tabular}} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Scenario} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Ground} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Visible\\Satellite\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Invisible\\Satellite\end{tabular} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Computing\\~Resource\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Transmission\\~Resource\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Transmission\\~Path\end{tabular}}  \\ 
	\hline
	\cite{8387798,8663968,8713498}                                                                    & \multirow{3}{*}{Tree}                                                                                                                                      & Cellular                                                       & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{3-9}
	\cite{9447257,8877759}                                                                            &                                                                                                                                                            & UAV                                                            & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{3-9}
	\cite{8936886}                                                                            &                                                                                                                                                            & IoT                                                            & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\hline
	\cite{9552467}                                                                                    & \multirow{3}{*}{Tree}                                                                                                                                      & \multirow{4}{*}{Satellite}                                     & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{4-9}
	\cite{9383778,9515574,inproceedings,9148261}                                                      &                                                                                                                                                            &                                                                &                                                              & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{4-9}
	\cite{ZHAO202294,9344666}                                                                         &                                                                                                                                                            &                                                                & \checkmark                                                   & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-2}\cline{4-9}
	\cite{9651919,7805169,9013462}                                                                    & Mesh                                                                                                                                                       &                                                                & \checkmark                                                   &                                                                                                 &                                                                                                   &                                                                                                                                                         & \checkmark                                                                                                                                                 & \checkmark                                                                                                                                              \\ 
	\hline
	\rowcolor[rgb]{0.812,0.835,0.918} Our work                                                        & Mesh                                                                                                                                                       & Satellite                                                      & \checkmark                                                   & \checkmark                                                                                      & \checkmark                                                                                        & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 & \checkmark                                                                                                                                              \\
	\hline
\end{tabular}

==> 1-Latex - arxiv/table2.tex <==
\arrayrulecolor{black}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
	\hline
	\rowcolor[rgb]{0.812,0.835,0.918} {\cellcolor[rgb]{0.812,0.835,0.918}}                           & {\cellcolor[rgb]{0.812,0.835,0.918}}                            & {\cellcolor[rgb]{0.812,0.835,0.918}}                           & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                      & \multicolumn{3}{c|}{Offloading Target}                                                                                                                                                                                                                             & \multicolumn{3}{c|}{Optimization}                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ 
	\hhline{|>{\arrayrulecolor[rgb]{0.812,0.835,0.918}}---->{\arrayrulecolor{black}}------|}
	\rowcolor[rgb]{0.812,0.835,0.918} {\cellcolor[rgb]{0.812,0.835,0.918}}                           & {\cellcolor[rgb]{0.812,0.835,0.918}}                            & {\cellcolor[rgb]{0.812,0.835,0.918}}                           & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                      & {\cellcolor[rgb]{0.812,0.835,0.918}}                         & \multicolumn{2}{c|}{Space}                                                                                                                                                                          & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                   & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                      & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                   \\ 
	\hhline{|>{\arrayrulecolor[rgb]{0.812,0.835,0.918}}----->{\arrayrulecolor{black}}-->{\arrayrulecolor[rgb]{0.812,0.835,0.918}}--->{\arrayrulecolor{black}}|}
	\rowcolor[rgb]{0.812,0.835,0.918} \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Category} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Reference} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Scenario} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Network\\Architecture\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Ground} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Visible\\Satellite\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Invisible\\Satellite\end{tabular} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Computing\\Resource\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Transmission\\Resource\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Transmission\\Path\end{tabular}}  \\ 
	\hline
	1                                                                                                & \cite{9651919,7805169,9013462}                                  & \multirow{4}{*}{Satellite}                                     & Mesh                                                                                                                                                      & \checkmark                                                   &                                                                                                 &                                                                                                   &                                                                                                                                                        & \checkmark                                                                                                                                                & \checkmark                                                                                                                                             \\ 
	\cline{1-2}\cline{4-10}
	2                                                                                                & \cite{9148261}                                                  &                                                                & \multirow{6}{*}{Tree}                                                                                                                                     &                                                              & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                             &                                                                                                                                                           &                                                                                                                                                        \\ 
	\cline{1-2}\cline{5-10}
	\multirow{2}{*}{3}                                                                               & \cite{9383778,9515574}                                  &                                                                &                                                                                                                                                           &                                                              & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                             & \checkmark                                                                                                                                                &                                                                                                                                                        \\ 
	\cline{2-2}\cline{5-10}
	& \cite{9344666,9793590}                                                  &                                                                &                                                                                                                                                           & \checkmark                                                   & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                             & \checkmark                                                                                                                                                &                                                                                                                                                        \\ 
	\cline{1-3}\cline{5-10}
	\multirow{3}{*}{4}                                                                               & \cite{8387798,8663968,8713498}                                  & Cellular                                                       &                                                                                                                                                           & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                             & \checkmark                                                                                                                                                &                                                                                                                                                        \\ 
	\cline{2-3}\cline{5-10}
	& \cite{9447257,8877759}                                          & UAV                                                            &                                                                                                                                                           & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                             & \checkmark                                                                                                                                                &                                                                                                                                                        \\ 
	\cline{2-3}\cline{5-10}
	& \cite{8936886}                                          & IoT                                                            &                                                                                                                                                           & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                             & \checkmark                                                                                                                                                &                                                                                                                                                        \\ 
	\hline
	\rowcolor[rgb]{0.812,0.835,0.918} \multicolumn{2}{|c|}{ Our work}                                                                                                  & Satellite                                                      & Mesh                                                                                                                                                      & \checkmark                                                   & \checkmark                                                                                      & \checkmark                                                                                        & \checkmark                                                                                                                                             & \checkmark                                                                                                                                                & \checkmark                                                                                                                                             \\
	\hline
\end{tabular}

==> Sentence.tex <==
In addition to industry growing interest, academic
researchers have eagerly jumped into the development of small
satellites.

However, despite of great potential of FSO communication, its performance is limited by the adverse effects (viz., absorption, scattering, and turbulence) of the atmospheric channel. Out of these three effects, the atmospheric turbulence is a major challenge that may lead to serious degradation in the bit error rate performance of the system and make the communication link infeasible~\cite{7553489}. 

RS techniques have opened a door to helping people widen their ability to understand the earth [1], [2]. In fact, RS techniques are becoming more and more important in data-collection tasks. Information technology companies depend on RS to update their location-based services [3], [4]. Google Earth employs high-resolution (HR) RS images to provide vivid pictures of the earth s surface. Governments have also utilized RS for a variety of public services, from weather reporting to traffic monitoring [5] [7]. Nowadays, one cannot imagine a life without RS. Recent years have even witnessed a boom in RS satellites, providing for the first time an extremely large number of geographical images of nearly every corner of the earth s  surface [8]. Data warehouses of RS images are increasing daily, including images with different spectral and spatial resolutions [9], [10]. ~\cite{7486259}

==> table2-new.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|c|} 
	\hline
	\rowcolor[rgb]{0.812,0.835,0.918} {\cellcolor[rgb]{0.812,0.835,0.918}}                            & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                       & {\cellcolor[rgb]{0.812,0.835,0.918}}                           & \multicolumn{3}{c|}{Offloading Target}                                                                                                                                                                                                                             & \multicolumn{3}{c|}{Optimization}                                                                                                                                                                                                                                                                                                                                                                                                                                              \\ 
	\hhline{|>{\arrayrulecolor[rgb]{0.812,0.835,0.918}}--->{\arrayrulecolor{black}}------|}
	\rowcolor[rgb]{0.812,0.835,0.918} {\cellcolor[rgb]{0.812,0.835,0.918}}                            & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                       & {\cellcolor[rgb]{0.812,0.835,0.918}}                           & {\cellcolor[rgb]{0.812,0.835,0.918}}                         & \multicolumn{2}{c|}{Space}                                                                                                                                                                          & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                    & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                       & {\cellcolor[rgb]{0.812,0.835,0.918}}                                                                                                                    \\ 
	\hhline{|>{\arrayrulecolor[rgb]{0.812,0.835,0.918}}---->{\arrayrulecolor{black}}-->{\arrayrulecolor[rgb]{0.812,0.835,0.918}}--->{\arrayrulecolor{black}}|}
	\rowcolor[rgb]{0.812,0.835,0.918} \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Reference} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Network\\~Architechture\end{tabular}} & \multirow{-3}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Scenario} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}Ground} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Visible\\Satellite\end{tabular} & \begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Invisible\\Satellite\end{tabular} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Computing\\~Resource\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Transmission\\~Resource\end{tabular}} & \multirow{-2}{*}{{\cellcolor[rgb]{0.812,0.835,0.918}}\begin{tabular}[c]{@{}>{\cellcolor[rgb]{0.812,0.835,0.918}}c@{}}Transmission\\~Path\end{tabular}}  \\ 
	\hline
	\cite{8387798,8663968,8713498}                                                                    & \multirow{3}{*}{Tree}                                                                                                                                      & Cellular                                                       & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{3-9}
	\cite{9447257,8877759}                                                                            &                                                                                                                                                            & UAV                                                            & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{3-9}
	\cite{8936886}                                                                            &                                                                                                                                                            & IoT                                                            & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\hline
	\cite{9552467}                                                                                    & \multirow{3}{*}{Tree}                                                                                                                                      & \multirow{4}{*}{Satellite}                                     & \checkmark                                                   &                                                                                                 &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{4-9}
	\cite{9383778,9515574,inproceedings,9148261}                                                      &                                                                                                                                                            &                                                                &                                                              & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-1}\cline{4-9}
	\cite{ZHAO202294,9344666}                                                                         &                                                                                                                                                            &                                                                & \checkmark                                                   & \checkmark                                                                                      &                                                                                                   & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 &                                                                                                                                                         \\ 
	\cline{1-2}\cline{4-9}
	\cite{9651919,7805169,9013462}                                                                    & Mesh                                                                                                                                                       &                                                                & \checkmark                                                   &                                                                                                 &                                                                                                   &                                                                                                                                                         & \checkmark                                                                                                                                                 & \checkmark                                                                                                                                              \\ 
	\hline
	\rowcolor[rgb]{0.812,0.835,0.918} Our work                                                        & Mesh                                                                                                                                                       & Satellite                                                      & \checkmark                                                   & \checkmark                                                                                      & \checkmark                                                                                        & \checkmark                                                                                                                                              & \checkmark                                                                                                                                                 & \checkmark                                                                                                                                              \\
	\hline
\end{tabular}
